How Data Inter-connectivity Shapes LLMs Unlearning: A Structural Unlearning Perspective

While unlearning knowledge from large language models (LLMs) is receiving increasing attention, one important aspect remains unexplored. Existing approaches and benchmarks assume data points to-be-forgotten are independent, ignoring their inter-connectivity - a fundamental characteristic of real-world data structures. In this paper, we propose PISTOL, a method for compiling structural datasets. PISTOL leverages the inherently structured nature of contractual relationships, offering several key benefits. First, it enables insights into the impact of structural data on unlearning effectiveness. Second, it provides precise and concise ground truths for clearer evaluation. Third, its attribute generation does not require input from pre-trained LLMs, mitigating confounding risks. Leveraging datasets synthesized using PISTOL, we demonstrate how data inter-connectivity impacts LLM unlearning. Specifically, (a) in both the pre-trained and fine-tuned models, unlearning difficulty increases as data inter-connectivity grows, (b) there is a positive correlation between the density of the knowledge graph and unlearning difficulty, and (c) when the to-be-forgotten data is skewed towards one domain, balancing retaining performance across all domains is challenging.

==> 4_new_unlearning_tasks.tex <==
\section{New Unlearning Considerations} \label{sec:forgettype}
{\color{blue}
Building on the concept of structural LLM unlearning introduced in Section \ref{sec:intro}, we categorize key structural unlearning considerations in this section, highlighting their real-world applications and significance.
}

\paragraph{RQ1: How does data inter-connectivity impact the unlearning performance?}
{\color{blue}
Previous studies on LLM unlearning have primarily focused on forgetting independent data points, overlooking the impact of interconnected data. However, in real-world scenarios, data points function as interconnected parcels of information, forming edges between subjects in knowledge graphs. Some entities naturally appear more frequently across data points than others, highlighting the need for structural LLM unlearning. An effective unlearning algorithm must robustly handle unlearning requests for subjects with varying levels of inter-connectivity while minimizing the need for manual intervention, such as extensive learning rate tuning.
}

\paragraph{RQ2: How does unlearning a specific data type affect the retained model’s performance on the same versus different data types?} 
%
This question highlights a real need, as unlearning requests may specifically target certain data types (e.g. one of the two contract types in Dataset 1) rather than encompassing a mix of all data types, as reflected by their proportional representation in the training set. For the first time, we investigate how such targeted unlearning affects outcomes, particularly examining whether it leads to uneven performance degradation on the retained data of both the same and different types.


==> fig_tab/99_table_quantity.tex <==
%quantity big table
\begin{table}[h!]
\centering
\captionsetup{font=small,labelfont=bf}
\caption{Unlearning results with different quantity}
\label{tab:quantity}
\scalebox{0.56}{
\begin{tabular}{ll | ccc |ccc|ccc}
\toprule
\multicolumn{2} {c} {\textbf{Llama2-7B}} & \multicolumn{3} {|c|} {\textbf{Rouge Score}}& \multicolumn{3} {|c|} {\textbf{MRR}} & \multicolumn{3} {|c} {\textbf{Top Hit Ratio}} \\
 \midrule
{\textbf{Forget}} & {\textbf{Forget}}   & {\textbf{Forget}} & {\textbf{Retained}} & {\textbf{Factual}} &{\textbf{Forget}} & {\textbf{Retained}} & {\textbf{Factual}}&{\textbf{Forget}} & {\textbf{Retained}} & {\textbf{Factual}}\\
{\textbf{Edge}} & {\textbf{Method}} & {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}}& {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}}& {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}}\\

\midrule
\multirow{4}{*}{\textbf{AC}} & GA & 0.267 ± 0.029 & 0.805 ± 0.005 & 0.846 ± 0.010 & 
0.179 ± 0.001 & 0.271 ± 0.004 & 0.251 ± 0.011 & 
0.606 ± 0.004 & 0.735 ± 0.006 & 0.579 ± 0.008 
\\

& GD  & 0.283 ± 0.029 & 0.920 ± 0.005 & 0.850 ± 0.004 & 
0.168 ± 0.002 & 0.261 ± 0.002 & 0.250 ± 0.005 &
0.590 ± 0.009 & 0.728 ± 0.008 & 0.581 ± 0.003  
\\

& KL   & 0.505 ± 0.256 & 0.793 ± 0.165 & 0.955 ± 0.005 &
0.357 ± 0.031 & 0.407 ± 0.044 & 0.206 ± 0.002 &
0.694 ± 0.073 & 0.784 ± 0.047 & 0.568 ± 0.002 
\\

& DPO    & 0.242 ± 0.000 & 0.933 ± 0.008 & 0.881 ± 0.001 &
0.159 ± 0.001 & 0.277 ± 0.001 & 0.221 ± 0.001 &
0.425 ± 0.003 & 0.658 ± 0.009 & 0.576 ± 0.001 
\\
%\addlinespace
\midrule
\multirow{4}{*}{\textbf{AC AC\textsubscript{2} AC\textsubscript{3}}} & GA & 0.000 ± 0.000 & 0.000 ± 0.000 & 0.003 ± 0.006 & 
0.026 ± 0.044 & 0.025 ± 0.044 & 0.004 ± 0.008 & 
0.107 ± 0.185 & 0.108 ± 0.186 & 0.045 ± 0.075 
\\

& GD  & 0.134 ± 0.037 & 0.760 ± 0.025 & 0.795 ± 0.024 & 
0.129 ± 0.013 & 0.221 ± 0.005 & 0.319 ± 0.024 &
0.327 ± 0.022 & 0.455 ± 0.026 & 0.574 ± 0.006  
\\

& KL   & 0.003 ± 0.005 & 0.014 ± 0.025 & 0.529 ± 0.359 &
0.105 ± 0.085 & 0.108 ± 0.087 & 0.067 ± 0.084 &
0.193 ± 0.046 & 0.189 ± 0.066 & 0.314 ± 0.161 
\\

& DPO    & 0.075 ± 0.025 & 0.987 ± 0.003 & 0.891 ± 0.003 &
0.130 ± 0.030 & 0.295 ± 0.001 & 0.232 ± 0.003 &
0.431 ± 0.031 & 0.739 ± 0.005 & 0.577 ± 0.002 
\\

\bottomrule
\toprule
\multicolumn{2} {c} {\textbf{Mistral-7B}} & \multicolumn{3} {|c|} {}& \multicolumn{3} {|c|} {} & \multicolumn{3} {|c} {}\\
\midrule
\multirow{4}{*}{\textbf{AC}} & GA & 0.184 ± 0.058 & 0.890 ± 0.010 & 0.916 ± 0.004 & 
0.134 ± 0.054 & 0.236 ± 0.004 & 0.513 ± 0.006 & 
0.252 ± 0.079 & 0.597 ± 0.025 & 0.755 ± 0.008 
\\

& GD  & 0.261 ± 0.077 & 0.959 ± 0.010 & 0.929 ± 0.004 & 
0.149 ± 0.006 & 0.266 ± 0.005 & 0.505 ± 0.004 &
0.293 ± 0.047 & 0.635 ± 0.016 & 0.748 ± 0.003  
\\

& KL   & 0.739 ± 0.010 & 0.968 ± 0.008 & 0.966 ± 0.003 &
0.246 ± 0.002 & 0.279 ± 0.008 & 0.700 ± 0.012 &
0.727 ± 0.019 & 0.757 ± 0.008 & 0.877 ± 0.004 
\\

& DPO    & 0.000 ± 0.000 & 0.949 ± 0.004 & 0.949 ± 0.003 &
0.018 ± 0.001 & 0.269 ± 0.004 & 0.598 ± 0.001 &
0.125 ± 0.000 & 0.676 ± 0.001 & 0.820 ± 0.001 
\\

\midrule
\multirow{4}{*}{\textbf{AC AC\textsubscript{2} AC\textsubscript{3}}} & 
GA & 0.000 ± 0.000 & 0.000 ± 0.000 & 0.000 ± 0.000 & 
0.000 ± 0.000 & 0.000 ± 0.000 & 0.001 ± 0.000 & 
0.000 ± 0.000 & 0.000 ± 0.000 & 0.000 ± 0.000 
\\

& GD  & 0.000 ± 0.000 & 0.020 ± 0.009 & 0.069 ± 0.034 & 
0.000 ± 0.000 & 0.035 ± 0.002 & 0.190 ± 0.027 &
0.000 ± 0.000 & 0.173 ± 0.010 & 0.445 ± 0.022  
\\

& KL   & 0.000 ± 0.000 & 0.012 ± 0.010 & 0.000 ± 0.000 &
0.049 ± 0.048 & 0.080 ± 0.027 & 0.000 ± 0.000 &
0.173 ± 0.159 & 0.000 ± 0.000 & 0.305 ± 0.041 
\\

& DPO    & 0.005 ± 0.002 & 0.003 ± 0.003 & 0.304 ± 0.009 &
0.009 ± 0.004 & 0.006 ± 0.001 & 0.163 ± 0.019 &
0.024 ± 0.002 & 0.034 ± 0.002 & 0.428 ± 0.020 
\\

\bottomrule
\end{tabular}
}

\end{table}


==> fig_tab/structured_tofu.tex <==
\begin{table}[h]
\centering
%\captionsetup{font=small,labelfont=bf}
\captionsetup{font=scriptsize,labelfont=bf}
\caption{(Structured TOFU 2) Unlearning results on the newly structured TOFU dataset, which introduces additional relationships between authors from the most commonly appearing country (i.e., the U.S.). Each unlearning U.S. author is connected to 8 other U.S. authors by country of birth (represented by 1 QA pair) and to 5 other U.S. authors through personal relationships (represented by 10 QA pairs). In contrast, the author from a country with only a single representative is completely independent of other authors. The table presents the average unlearning results for three randomly selected U.S. authors (who represent highly interconnected nodes in the graph) compared to those from countries with a single author (who represent lowly interconnected nodes in the graph).}
\label{tab:tofu2}
\scalebox{0.5}{

\begin{tabular}{ll |cc |cc |cc}
\toprule
{\textbf{Country}} & {\textbf{Methods}} & \multicolumn{2} {|c|} {\textbf{Rouge Score}}& \multicolumn{2} {|c|} {\textbf{MRR}} & 
\multicolumn{2} {|c} {\textbf{Top Hit Ratio}} \\
 \midrule
\multicolumn{2} {c|} {\textbf{Llama2-7B}} & {\textbf{Forget}} & {\textbf{Retained}} & {\textbf{Forget}} & {\textbf{Retained}} &{\textbf{Forget}} & {\textbf{Retained}}\\
 &  & {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}}& {\textbf{Set}} & {\textbf{Set}}\\

\midrule
\multirow{4}{0em}{\textbf{USA}} & GA & 0.368 ± 0.021 & 0.734 ± 0.022 & 0.074 ± 0.012 & 0.414 ± 0.022 & 0.203 ± 0.019 & 0.534 ± 0.021 \\
& GD & 0.393 ± 0.016 & 0.784 ± 0.009 & 0.087 ± 0.004 & 0.457 ± 0.008 & 0.218 ± 0.009 & 0.576 ± 0.009 \\
& KL & 0.652 ± 0.023 & 0.738 ± 0.019 & 0.157 ± 0.014 & 0.353 ± 0.013 & 0.358 ± 0.012 & 0.521 ± 0.013 \\
& DPO & 0.138 ± 0.013 & 0.730 ± 0.015 & 0.036 ± 0.007 & 0.455 ± 0.010 & 0.150 ± 0.014 & 0.595 ± 0.010 \\

\midrule

\multirow{4}{*}{\shortstack[l]{\textbf{Country w/} \\\textbf{1 Author}}} & GA & 0.298 ± 0.005 & 0.811 ± 0.023 & 0.043 ± 0.006 & 0.486 ± 0.017 & 0.149 ± 0.013 & 0.606 ± 0.017 \\
& GD & 0.352 ± 0.015 & 0.907 ± 0.018 & 0.043 ± 0.007 & 0.558 ± 0.014 & 0.151 ± 0.018 & 0.674 ± 0.012 \\
& KL & 0.624 ± 0.035 & 0.719 ± 0.020 & 0.131 ± 0.024 & 0.342 ± 0.020 & 0.324 ± 0.031 & 0.508 ± 0.017 \\
& DPO & 0.144 ± 0.022 & 0.801 ± 0.010 & 0.025 ± 0.002 & 0.493 ± 0.009 & 0.143 ± 0.011 & 0.624 ± 0.007 \\
\bottomrule


\end{tabular}
}
\end{table}

==> fig_tab/tofu_country.tex <==
\begin{table}[h]
\centering
%\captionsetup{font=small,labelfont=bf}
\captionsetup{font=scriptsize,labelfont=bf}
\caption{(Structured TOFU 1) Unlearning results on the newly constructed structured TOFU dataset, which introduces entity relationship in terms of the country of birth. The U.S. has the highest representation with 9 out of 200 authors in the TOFU dataset, while countries like Zimbabwe and Portugal have the lowest, each with only one author. The table shows the average unlearning results for three randomly selected U.S. authors (who represent highly interconnected nodes in the graph) compared to those from countries with a single author (who represent lowly interconnected nodes in the graph).}
\label{tab:tofu1}
\scalebox{0.5}{

\begin{tabular}{ll |cc |cc |cc}
\toprule
{\textbf{Country}} & {\textbf{Methods}} & \multicolumn{2} {|c|} {\textbf{Rouge Score}}& \multicolumn{2} {|c|} {\textbf{MRR}} & 
\multicolumn{2} {|c} {\textbf{Top Hit Ratio}} \\
 \midrule
\multicolumn{2} {c|} {\textbf{Llama2-7B}} & {\textbf{Forget}} & {\textbf{Retained}} & {\textbf{Forget}} & {\textbf{Retained}} &{\textbf{Forget}} & {\textbf{Retained}}\\
 &  & {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}} & {\textbf{Set}}& {\textbf{Set}} & {\textbf{Set}}\\

\midrule
\multirow{4}{0em}{\textbf{USA}} & GA & 0.374 ± 0.017 & 0.838 ± 0.025 & 0.049 ± 0.011 & 0.493 ± 0.015 & 0.180 ± 0.012 & 0.603 ± 0.015 \\

& GD  & 0.394 ± 0.027 & 0.899 ± 0.013 & 0.058 ± 0.005 & 0.543 ± 0.012 & 0.189 ± 0.011 & 0.654 ± 0.011 \\

& KL  & 0.704 ± 0.020 & 0.797 ± 0.020 & 0.171 ± 0.008 & 0.409 ± 0.029 & 0.350 ± 0.055 & 0.567 ± 0.028 \\

& DPO & 0.163 ± 0.018 & 0.831 ± 0.008 & 0.023 ± 0.003 & 0.526 ± 0.006 & 0.150 ± 0.004 & 0.663 ± 0.005 \\

\midrule

\multirow{4}{*}{\shortstack[l]{\textbf{Country w/} \\\textbf{1 Author}}} & GA & 0.353 ± 0.022 & 0.877 ± 0.018 & 0.066 ± 0.004 & 0.515 ± 0.013 & 0.165 ± 0.014 & 0.624 ± 0.014 \\

& GD  & 0.350 ± 0.009 & 0.917 ± 0.013 & 0.066 ± 0.004 & 0.545 ± 0.013 & 0.171 ± 0.057 & 0.657 ± 0.014 \\

& KL  & 0.661 ± 0.037 & 0.740 ± 0.028 & 0.186 ± 0.020 & 0.354 ± 0.038 & 0.366 ± 0.025 & 0.518 ± 0.034 \\

& DPO & 0.111 ± 0.011 & 0.814 ± 0.016 & 0.021 ± 0.005 & 0.509 ± 0.018 & 0.139 ± 0.022 & 0.645 ± 0.015 \\

\bottomrule

\end{tabular}
\label{tab:tofu_country}
}
\end{table}

